ArcheType: A Novel Framework for Open-Source Column Type Annotation using Large Language Models

Existing deep-learning approaches to semantic column type annotation (CTA) have important shortcomings: they rely on semantic types which are fixed at training time; require a large number of training samples per type and incur large run-time inference costs; and their performance can degrade when evaluated on novel datasets, even when types remain constant. Large language models have exhibited strong zero-shot classification performance on a wide range of tasks and in this paper we explore their use for CTA. We introduce ArcheType, a simple, practical method for context sampling, prompt serialization, model querying, and label remapping, which enables large language models to solve CTA problems in a fully zero-shot manner. We ablate each component of our method separately, and establish that improvements to context sampling and label remapping provide the most consistent gains. ArcheType establishes a new state-of-the-art performance on zero-shot CTA benchmarks (including three new domain-specific benchmarks which we release along with this paper), and when used in conjunction with classical CTA techniques, it outperforms a SOTA DoDuo model on the fine-tuned SOTAB benchmark. Our code is available at https://github.com/penfever/ArcheType.

==> figures/archetype-datasets.tex <==
   \begin{tcolorbox}[colback=white!97!black,colframe=brown!98!black]
    \begin{small}
    \begin{verbatim}
SOTAB-27
\end{verbatim}
 \end{small}
 \tcblower
  \begin{small}
 \begin{verbatim}
CREATIVE WORK : "What to Expect When You’re Expecting 
(4th Edition)", "The Better Baby Book: How to Have..."
PERSON: "Otoo, Sharon Dodua", "Danysz, Magda"
PRODUCT: "SKL-200", "1160"
 \end{verbatim}
 \end{small}
\end{tcolorbox}

\begin{tcolorbox}[colback=white!94!black,colframe=brown!95!black]
    \begin{small}
    \begin{verbatim}
D4-20
\end{verbatim}
 \end{small}
 \tcblower
  \begin{small}
 \begin{verbatim}
EDUCATIONAL ORGANIZATION: "The Global Learning Collab", 
"P.S. 057 Hubert H. Humphrey"
REGION IN THE BRONX: "Bathgate", "Crotona Park East"
CITY AGENCY (FULL): "Mayor's Office of Media 
and Entertainment (MOME)", "Department of Design 
and Construction (DDC)"
 \end{verbatim}
 \end{small}
\end{tcolorbox}
\begin{tcolorbox}
[colback=white!91!black,colframe=brown!85!black]
    \begin{small}
    \begin{verbatim}
Amstr-56
\end{verbatim}
 \end{small}
 \tcblower
  \begin{small}
 \begin{verbatim}
ARTICLE FROM PA: "REDLANDS, Feb. 6.-The Casa Iona hotel 
was last evening the scene..."
NEWSPAPER: "The Nome nugget.", "The Arizona champion."
 \end{verbatim}
 \end{small}
\end{tcolorbox}
\begin{tcolorbox}
[colback=white!88!black,colframe=brown!75!black]
    \begin{small}
    \begin{verbatim}
Pubchem-20
\end{verbatim}
 \end{small}
 \tcblower
  \begin{small}
 \begin{verbatim}
MOLECULAR FORMULA: "C10H30Cl4O2Si4", "C43H75NO10S"
DISEASE: "Myofibrillar myopathy, filamin C-related"
 \end{verbatim}
 \end{small}
\end{tcolorbox}
%\vspace{-.3cm}

==> figures/archetype-six-prompts-reduced.tex <==
\centering
\begin{tcolorbox}[colback=yellow!25!white,colframe=white!25!black]
\begin{small}
%\begin{verbatim}
\textbf{C:} \texttt{"For the following table column, select a schema.org 
type annotation from <CLASSNAMES>. Input column: 
<CONTEXT>. Output: "}

\textbf{K:} \texttt{"Answer the question based on the task below. If the 
question cannot be answered using the information 
provided, answer with "I don't know". Task: Classify 
the column given to you into only one of these types: 
<CLASSNAMES>. Input column: <CONTEXT>. Type: "}

\textbf{I:} \texttt{"Here is a column from a table: <CONTEXT>. 
Please select the class from that best describes the 
column, from the following options. Options: 
<CLASSNAMES> Response: "}

\textbf{S:} \texttt{"Pick the column's class. Column: <CONTEXT>. 
Classes: <CLASSNAMES>. Output: "}

\textbf{N:} \texttt{"Pick the column's class. I mean if you want to. It 
would be cool, I think. Anyway, give it a try, I guess? 
Here's the column itself! <CONTEXT>. And, um, 
here are some column names you could pick from ... 
<CLASSNAMES>. Ok, go ahead! "}

\textbf{B:} \texttt{"INSTRUCTION: Select the {option | category} 
which best {describes | matches} the input. 
INPUT: <CONTEXT> OPTION: <CLASSNAMES> ANSWER:"}
%\end{verbatim}
\end{small}
\end{tcolorbox}

==> tables/OLD-archetype-table.tex <==
\begin{table*}[!t]
    \centering
    %\resizebox{0.8\linewidth}{!}
    {
        \begin{tabular}{l l l l l}
        \toprule
            \parbox{2cm}{Model Name} & \parbox{2cm}{Dataset (Train)} & \parbox{2cm}{Dataset (Eval)} & \parbox[c]{2cm}{Micro-F1} & \parbox{2cm}{Context Req'd} \\ 
            \midrule
            \multicolumn{5}{l}{\textit{Fine-Tuned}} \\

            DoDuo & VizNet + SOTAB-91 & SOTAB-91   & \textbf{84.82} $\pm 0.6$     & Entire Table                                                                                    \\
            ArcheType-LLAMA & LLAMA + SOTAB-91  & SOTAB-91    & \textbf{84.65} $\pm 0.6$   & 15 cross-col samples, stats, table name \\
            TURL & TURL-Tables + SOTAB-91 & SOTAB-91 & 78.96 $\pm 0.7$ & Entire Table \\
            \midrule
            \multicolumn{5}{l}{\textit{Zero-Shot}} \\ % this is your label
            ArcheType-T5 & Flan-PaLM & SOTAB-27 & \textbf{38.37} $\pm 0.7$    & 10 samples                                                                  \\
            DoDuo & VizNet & SOTAB-27 & 23.81 $\pm 0.7$    & Entire Table                                                                                    \\
            ArcheType-T5 & Flan-PaLM & D4Tables-20 & \textbf{61.1} $\pm 2.1$     & 5 samples                                                                 \\
            DoDuo & VizNet & D4Tables-20 & 32.2 $\pm 2.0$     & Entire Table     \\
            \bottomrule \\
        \end{tabular}}
        \caption{\sl\textbf{ArcheType achieves state-of-the-art zero-shot performance on CTA benchmarks. } \sl  Our context sampling method, paired with a variety of public and semi-public large language models, is able to achieve state-of-the-art zero-shot results compared to the best available pre-trained model (DoDuo), and performs identically (within the margin of error) when fine-tuned. In the above table, (FT) refers to fine tuning, (ZS) to zero-shot. Context req'd describes the amount of data required by the model; our method is more data-efficient than previous methods. \textbf{Boldface} indicates the best-performing model(s).}
        \label{tab:main-results}
\end{table*}

==> tables/archetype-arch-ablation.tex <==
\begin{tabular}{l l l l l}
    \parbox{2cm}{Model Name} & \parbox{2cm}{Dataset} & \parbox[c]{2cm}{Micro-F1} & \parbox{2cm}{Params} & \parbox{2cm}{Arch.} \\ 
    \midrule
    ArcheType-GPT-3.5 & SOTAB-27 & \textbf{63.3} $\pm 0.8$ & 175B (speculation) & Decoder-only (speculation)         \\
    ArcheType-UL2      & SOTAB-27 & 56.4 $\pm 0.8$ & 20B     & Encoder-decoder \\
    ArcheType-T5   & SOTAB-27 & 54.0 $\pm 0.8$ & 11B     & Encoder-decoder \\
    ArcheType-LLAMA2 & SOTAB-27 & 30.0 $\pm 0.7$ & 13B & Decoder-only \\
    ArcheType-OPT-IML   & SOTAB-27 & 24.7 $\pm 0.7$ & 30B     & Decoder-only    \\
    ArcheType-LLAMA1   & SOTAB-27 & 20.1 $\pm 0.6$ & 7B     & Decoder-only    \\
\end{tabular}

==> tables/archetype-method-compare.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\textbf{Method} & \textbf{CS} & \textbf{PS} & \textbf{MQ} & \textbf{LR} \\
ArcheType & Ours & C,K,I,S,N,B & T5, UL2, GPT & Cont + Res \\
Chorus~\cite{kayali2023chorus} & Random & C & GPT & Sim \\
Korini~\cite{korini2023column} & First & K & GPT & Manual
\end{tabular}%
}
